Avoiding Catastrophe in Online Learning by Asking for Help

Most learning algorithms with formal regret guarantees assume that all mistakes are recoverable and essentially rely on trying all possible behaviors. This approach is problematic when some mistakes are "catastrophic", i.e., irreparable. We propose an online learning problem where the goal is to minimize the chance of catastrophe. Specifically, we assume that the payoff in each round represents the chance of avoiding catastrophe in that round and try to maximize the product of payoffs (the overall chance of avoiding catastrophe) while allowing a limited number of queries to a mentor. We also assume that the agent can transfer knowledge between similar inputs. We first show that in general, any algorithm either queries the mentor at a linear rate or is nearly guaranteed to cause catastrophe. However, in settings where the mentor policy class is learnable in the standard online model, we provide an algorithm whose regret and rate of querying the mentor both approach 0 as the time horizon grows. Although our focus is the product of payoffs, we provide matching bounds for the typical additive regret. Conceptually, if a policy class is learnable in the absence of catastrophic risk, it is learnable in the presence of catastrophic risk if the agent can ask for help.

==> limitations.tex <==
\section{Limitations}\label{sec:limitations}

Our paper contains both positive and negative results. As such, our claim in this paper is not ``avoiding catastrophe is possible (or impossible) under assumptions X, Y, Z, and we argue that X, Y, Z hold''. Instead, we aim to understand \emph{the conditions} under which it is possible to avoid catastrophe. Our claim is ``avoiding catastrophe is possible under X, Y, Z, but impossible under A, B, C; we might sometimes expect X, Y, Z and sometimes expect A, B, C''. For example, some real-world instances might exhibit finite Natarajan dimension, while others might not. Our paper elucidates what to expect from either scenario.

The goal, then, is to make the gap between X, Y, Z and A, B, C as small as possible: to isolate the boundary of tractability. Our results suggest that the key factor determining tractability is the complexity of the mentor policy class. Our negative result (\Cref{thm:neg}) shows that a simple environment (bounded 1D state space, known uniform distribution over states, two actions) is not enough for tractability if the mentor policy class is complex. On the other hand, our primary positive result (\Cref{thm:pos-nd-final}) holds for quite general environments (unbounded $n$-dimensional state space, unknown arbitrary distribution over states, many actions), as long as the mentor policy class is simple.

One weakness of \Cref{thm:pos-nd-final} is the dependence of the query bound on the number of actions. We think this can be significantly reduced or eliminated, possibly with additional mild assumptions. More broadly, the assumptions of (1) only caring about catastrophe and (2)  i.i.d. states significantly limit the real-world applicability of our algorithm. In future work, we hope to extend this result to general MDPs.

Our secondary positive result (\Cref{thm:simple-final}) also suggests that mentor policy complexity could be the key factor determining tractability. However, it has the drawback that the number of segments in the mentor policy is a less established measure of complexity than the well-studied notion of Natarajan dimension. In our opinion, the more serious limitation is the restriction to a 1D state space. Although \Cref{thm:simple-final} does permit adversarial state sequences, we feel that \Cref{thm:pos-nd-final} does a better overall job of isolating the boundary of tractability.





==> no_local_gen.tex <==
\section{Without local generalization}

The following three definitions can be found in Section 2.2 of \cite{hanneke2014active}.
\begin{definition}
\label{def:disagree}
The \emph{disagreement region} of a policy class $\Pi$ is $\dis(\Pi) = \{s \in S: \exists \pi_1, \pi_2 \in \Pi \text{ s.t. } \pi_1(s) \ne \pi_2(s)\}$.
\end{definition}

\begin{definition}\label{def:ball}
Given a policy class $\Pi$, distribution $\D$, and $\ep > 0$, let $B(\Pi,\D, \ep) = \{\pi \in \Pi: \Pr_{s \sim \D}[\pi(s) \ne \pi^m(s)] \le \ep\}$. For brevity, we usually write $B(\ep) = B(\Pi, \D, \ep)$.
\end{definition}

\begin{definition}
\label{def:disagree-coeff}
The \emph{disagreement coefficient} of a policy class $\Pi$, distribution $\D$, and $\ep > 0$ is
\[
\theta(\Pi, \D, \ep) = \max\left(1,\ \sup_{\ep' > \ep} \frac{\Pr_{s \sim \D}[s \in B(\ep')]}{\ep'}\right)
\]
We usually write $\theta(\ep) = \theta(\Pi, \D, \ep)$ for brevity.
\end{definition}

Note that $\ep_1\ge \ep_2$ implies $\theta(\ep_1) \le \theta(\ep_2)$, since for $\ep_2$ we are taking the supremum over a strictly smaller range. We also have the following useful property:

\begin{lemma}[Corollary 7.2 in \cite{hanneke2014active}]
\label{lem:dis-monotone}
If $\ep > 0$ and $x > 1$, then $\theta(\ep/x) \le x \theta(\ep)$.
\end{lemma}

\begin{algorithm}[tb]
\centering
\begin{algorithmic}[1]
\Function{CAL}{policy class $\Pi$}
\State $\tilpi \gets \Pi$
\For{$t$ \textbf{from} $1$ \textbf{to} $T$} 
    \If{$s_t \in \dis(\tilpi)$}
        \State Query and observe $\pi^m(s_t)$
        \State $\tilpi \gets \{\pi \in \tilpi: \pi(s_t) = \pi^m(s_t)\}$
    \Else
        \State Take action $\pi(s_t)$ for an arbitrary $\pi \in \tilpi$
    \EndIf
\EndFor
\EndFunction
\end{algorithmic}
\caption{caption me.}
\label{alg:cal}
\end{algorithm}

\begin{definition}
\label{def:consistent}
Given a policy class $\Pi$ and a set $X \subset S \times A$ of state-action pairs, let $\Pi_{|X} = \{\pi \in \Pi: \pi(s) = a\ \forall (s,a) \in X\}$.
\end{definition}

\begin{theorem}[Fundamental Theorem of PAC Learning \cite{shalev-shwartz_understanding_2014}]
Assume $\Pi$ has VC dimension $d$ and let $X \subset S \times A$ be a set of $m$ i.i.d. samples from $\D$. There exists a universal constant $c > 0$ such that if $m \ge \frac{c}{\ep}(d\log \ep^{-1} + \log \delta^{-1})$ for some $\ep,\delta \in (0,1)$, then with probability at least $1-\delta$, $\Pi_{|X} \subseteq B(\ep)$. \todo{phrasing}
\end{theorem}

\begin{corollary}
\label{cor:pac}
Assume $\Pi$ has VC dimension $d$ and let $X \subset S \times A$ be a set of $m$ i.i.d. samples from $\D$. There exists a universal constant $c > 0$ such that for any $\delta \in (0,1)$, with probability $1-\delta$, $\Pi_{|X} \subseteq B(\frac{c}{m}(d \log m + \log \delta^{-1}))$. 
\end{corollary}

\begin{proof}
Let $c$ be the constant from \Cref{thm:pac}; WLOG assume $c \ge 1$ (if \Cref{thm:pac} holds for some $c < 1$, it clearly also holds for $c \ge 1$). Let $\ep = \frac{c}{m}(d \log m + \log \delta^{-1})$. Since $\delta \in (0,1)$ and $c \ge 1$, we have $\ep \ge 1/m$ and thus $\log \ep^{-1} \le \log m$. Then
\begin{align*}
\frac{c}{\ep}(d\log \ep^{-1} + \log \delta^{-1}) =&\ \frac{m(d\log \ep^{-1} + \log \delta^{-1})}{d\log m + \log \delta^{-1}}\\
\le&\ \frac{m(d\log m + \log \delta^{-1})}{d\log m + \log \delta^{-1}}\\
=&\ m
\end{align*}
Therefore $m \ge \frac{c}{\ep}(d\log \ep^{-1} + \log \delta^{-1})$, so \Cref{thm:pac} implies that with probability at least $1-\delta$, $\Pi_{|X} \subseteq B(\ep) = B(\frac{c}{m}(d \log m + \log \delta^{-1}))$.
\end{proof}

\todo{Doesn't immediately work for Littlestone dim because e.g. for a finite hypothesis class, you can set it up so that each query only eliminates one possible classifier (whereas $Ldim(\Pi) = \log |\Pi|$}

For now we're assuming $\theta(\ep) \in O(1)$. This is satisfied, for example, for the class of thresholds on $[0,1]$ with the uniform distribution.

\begin{theorem}\label{thm:no-local-gen}
Let $A = \{0,1\}$, assume $\s$ is i.i.d. from some distribution $\D$, and assume $\theta(\ep) \in O(1)$. Then \Cref{alg:cal} satisfies
\begin{align*}
R_T =&\ 0\\
\E[Q_T] \in&\ O(d \log^2 T)
\end{align*}
\end{theorem}

\begin{proof}
For each $t \in [T]$, let $\tilpi_t$ be the value of $\tilpi$ at the end of time step $t$ and let $X_t = \cup_{i=1}^t \{(s_i, \pi^m(s_i)\}$. Then $\tilpi_t \subseteq \Pi_{|X_t}$. Also fix $\delta = 1/T^2$ and let $\ep_t = \frac{c}{t}(d \log t + \log \delta^{-1})$. Let $E_t$ be the event that $\Pi_{|X_t} \subseteq B(\ep_t)$ and let $E = \cap_{t=1}^T$. Then \Cref{cor:pac} implies that $\Pr[E_t] \ge 1-\delta$ for all $t \in [T]$, so $\Pr[E] \ge 1- T\delta$ by the union bound.

Now define random variables $z_1,\dots,z_T$ by $z_t = \bfone(s_t \in \dis(B(\ep_{t-1})))$ for $t > 1$ and $z_1 = 1$ (since $\ep_0$ is not well-defined). Under event $E$, $\tilpi_t \subseteq \Pi_{|X_t} \subseteq B(\ep_t)$ for all $t \in [T]$. Then for all $t > 1$ we have
\[
\Pr[t \in Q_T \mid E] = \Pr[s_t \in \dis(\tilpi_{t-1}) \mid E] \le \Pr[s_t \in \dis(B(\ep_{t-1})) \mid E] = \E[z_t \mid E]
\]
and so
\begin{align*}
\E[|Q_T| \mid E] \le&\ \sum_{t=1}^T \E[z_t \mid E]\\
=&\ 1 + \sum_{t=2}^T \Pr[s_t \in \dis(B(\ep_{t-1}))]\\
=&\ 1 + \sum_{t=2}^T \Pr_{s \sim \D}[s \in \dis(B(\ep_{t-1}))]\\
=&\ 1 + \sum_{t=1}^{T-1} \Pr_{s \sim \D}[s \in \dis(B(\ep_t))]\\
\le&\ 1+\sum_{t=1}^{T-1} \theta(\ep_t) \ep_t\\
\end{align*}
\todo{Justify $\D(\dis(B (\ep_t))) \le \theta(\ep_t)\ep_t$.}
For now let's say $\theta(\ep) \le c$. Then
\begin{align*}
\E[|Q_T| \mid E] \le&\ 1 + c \cdot \sum_{t=1}^T \frac{c}{t}(d \log t + 2 \log T)\\
\le&\ 1 + c^2 (d+2) \log T \sum_{t=1}^T \frac{1}{t}\\
\in&\ O(d \log^2 T)
\end{align*}

% Since $\ep_t = \frac{c}{t}(d \log t + 2 \log T) \ge \frac{c}{t}(d+2) \log t$
% For now assume $\theta(\ep) \in O(1)$. Then 
% If $\theta(\ep) \in o(1/\ep)$, then $0 = \lim_{\ep \to 0} \frac{\theta(\ep)}{1/\ep} = \lim_{\ep \to 0} \theta(\ep)\ep$. Since $\lim_{t\to\infty} \ep_t = 0$, we can switch the limit variable:
% \[
% \lim_{\ep \to 0} \theta(\ep)\ep = \lim_{t\to\infty} \theta(\ep_t) \ep_t = 0
% \]


% For all $t \in [T]$ we have $\ep_t \ge \ep_T$ and thus $\theta(\ep_t) \le \theta(\ep_T)$. Therefore
% \begin{align*}
% \le&\ 1+ c\, \theta(\ep_T) \sum_{t=1}^{T-1} \frac{1}{t}(d \log t + 2 \log \delta^{-1})\\
% \le&\ 1 + c\, \theta\left(\frac{c}{T}(d+2)\log T\right) (d+2)\log T \sum_{t=1}^{T-1} \frac{1}{t}
% \end{align*}
% Since 
% \in&\ O\left(d\, \theta(\ep_T) \log^2 T\right)
% \end{align*}
Since $|Q_T| \le T$ always, the total of total expectation implies that
\begin{align*}
\E[|Q_T|] =&\ \E[|Q_T| \mid E] \cdot \Pr[E] + \E[|Q_T| \mid \neg E] \cdot \Pr[\neg E]\\
\le&\ O(d \log^2 T) \cdot 1 + T \cdot T\delta\\
\in&\ O(d \log^2 T)
\end{align*}
as required.
\end{proof}
